An Empirical Exploration of Trust Dynamics in LLM Supply Chains

With the widespread proliferation of AI systems, trust in AI is an important and timely topic to navigate. Researchers so far have largely employed a myopic view of this relationship. In particular, a limited number of relevant trustors (e.g., end-users) and trustees (i.e., AI systems) have been considered, and empirical explorations have remained in laboratory settings, potentially overlooking factors that impact human-AI relationships in the real world. In this paper, we argue for broadening the scope of studies addressing `trust in AI' by accounting for the complex and dynamic supply chains that AI systems result from. AI supply chains entail various technical artifacts that diverse individuals, organizations, and stakeholders interact with, in a variety of ways. We present insights from an in-situ, empirical study of LLM supply chains. Our work reveals additional types of trustors and trustees and new factors impacting their trust relationships. These relationships were found to be central to the development and adoption of LLMs, but they can also be the terrain for uncalibrated trust and reliance on untrustworthy LLMs. Based on these findings, we discuss the implications for research on `trust in AI'. We highlight new research opportunities and challenges concerning the appropriate study of inter-actor relationships across the supply chain and the development of calibrated trust and meaningful reliance behaviors. We also question the meaning of building trust in the LLM supply chain.

==> sections/formalization.tex <==
%\section{Prelude: Overview of Relevant AI Supply Chain Components in Relation To Trust}%Identifying the Relevant Entities: the AI Stakeholders and AI Objects in the AI Supply Chain}


\subsection{Prelude: The entities making up trust relations}

\TODO{maybe stat directly by talking about the different trustors and trustees as is, and not only as a list of entities}

\TODO{think about how to account for system updates}

\fanny{From Agathe: can you review notations and validity of anything, and make suggestions on the formalization?}

In this section, based on our interviews and prior literature, we revise the set of entities that make up trust relations in the AI supply chain. Particularly, we account for a more complete understanding of the technical artifacts and human entities that constitute the AI supply chain. 
We do not describe in detail each individual modeling choice for space consideration. However, we point the reader to the primary considerations and main justifications for our choices.

\subsubsection{Technical Artifacts}
Technical artifacts are various components that are used across the AI supply chain in different phases of the AI system.  \TODO{from fanny: define the phases of the AI system}
It is important to model the relations between various technical artifacts, because it is now well-understood that an AI system is made up of different components at different phases of its life. With regard to trust, one might actually trust one component of the AI system but not the entire AI system itself. 
\fanny{Thus we define a technical artifact w.r.t. a given AI system?? Mathematically, do we have something in the likes of: 
\begin{quote}
    Let $TA$ the space of all tech artifacts and $S$ an AI system.
    Then there exists $TA_S = \{ta_1, \ldots, ta_m\} \subseteq TA$ the set of tech artifacts leveraged by $S$. 
    Let $T = \{\text{pretrained}, \text{in-use}, \text{other} \}$ the set of possible types [blabla].
    We define $\tau: TA \times S \to T$ the function mapping an artifact of an AI system to its type.
    We define $\mathcal{R}$ the binary relation connecting tech artifacts together such that $ta_1 \in TA_S$ is $\mathcal{R}$-related to $ta_2 \in TA_S$ iff $ta_1$ \textbf{impacts} $ta_2$.
    Thus, we can represent $S$ with the directed graph $(TA_S, \mathcal{R})$.
    Also, $\mathcal{R}$ is a transitive relation: [explain transitivity in plain language].
\end{quote}}
\TODO{from fanny: adjust "impacts"}

\framedtext{
\underline{\textbf{Formalization of the technical artifacts:}}
\begin{itemize}[leftmargin=*]
    \item 
    \item The space of technical artifacts: $TA$; individual artifacts: $ta\_x \in TA$
    \item \textbf{The type of the technical artifacts}: {$T\_TA: TA \times \{types\} \rightarrow True / False$}. 
    \begin{itemize}
        \item Constraints: Note that a technical artifact can only be associated with a single type.
        \item We propose the following types: \textit{pre-trained-AI-system, in-use-AI-system, other.} 
        \fanny{\textbf{ISSUE? do i misunderstand what you mean by pre-trained?} If we generically define $TA$--aka independently of AI system, we run into a contradiction of the above constraint. For example, i can use T5 as is for a given task with their template (type = in-use) but further fine-tune it for an other (type = pre-trained). Am i mistaken?}
        \agathe{yes, that's what i meant. i thought it's convenient because indeed one technical artifact can be used by different stakeholders in different ways} 
        \fanny{Ok! This means that we need to "fix" an AI system $S$ first and then we define tech artifact w.r.t. to $S$ so things work as expected. The math language above does that.}
    \end{itemize}
    \item \textbf{Relations between technical artifacts}:  $R\_TA: TA \times TA \rightarrow True / False$
    \begin{itemize}
        \item Meaning: This means that the first argument is a component of the second argument.
        \item Transitivity: This is a transitive relation (if $ta1 \in TA$, $ta2 \in TA$ and $ta3 \in TA$, and $R\_TA(ta1, ta2)$ and $R\_TA(ta2, ta3)$, then $R\_TA(ta1, ta3)$).
        \item This is not a symmetric relation, nor a reflexive relation.
        \item Constraints: There are a few natural constraints on this relation. 
        \begin{itemize}
            \item  Particularly, an AI system cannot be a component of a technical artifact of type ``other'' (e.g., an AI system cannot be the component of a dataset).         Note that a system can be the component of another system since some systems are made up of several concatenated AI models \cite{}. 
            \item There exists always at least one technical artifact of type ``other'' that composes an AI system.
        \end{itemize}
    \end{itemize}
\end{itemize}
}

We propose only the above types of technical artifacts, because this is the distinction that revealed most useful when investigating trust relations, and existing literature, e.g., on governance of AI systems \cite{}. Typically, one distinguishes between the pre-trained system that can be fine-tuned in various ways to create various in-use-AI-systems, that will be used to conduct different tasks.
When an in-use-system has been fine-tuned on a specific pre-trained-AI-system, we consider the second to be a component of the first (i.e., $R\_TA(pre-trained-AI-system, in-use-AI-system) = True$).
The technical artifacts of type ``other'' can be very diverse. On the side of the in-use-AI-system, one can think of the fine-tuned model, of the workflows for filtering the outputs of this model (e.g., for hate speech), for monitoring the outputs (e.g., for distribution shifts), and for updating the model. Common or distinct for the pre-trained-AI-system and in-use-AI-system, one can think of the software in which the AI model is integrated, the data used to train or evaluate it (e.g., the data is itself composed of several data samples and data annotations), the training scripts for the model, the various infrastructures needed, e.g., to store the data, to conduct the training computation, to host the AI system, etc.


\subsubsection{Human entities: Individual and Organizational Entities in relation to the Technical Artifacts}


We now define the individual and organizational entities.

\framedtext{
\textbf{\underline{Formalization of the human entities:}}
\begin{itemize}[leftmargin=*]
    \item The space of individual entities: $I$; with $i_x \in I$
    \item The space of organizational entities: $O$; with $o_x \in O$ \fanny{are inactive/dissolved org in this space?}
    \item \textbf{Relations between human entities}:
    \begin{itemize}
        \item \textbf{Role of an individual entity w.r.t an organizational entity}: $R\_IO\_role : I \times O \times type\_role\_IO \rightarrow True / False$    \\
The type the relation can take corresponds to the role of the individual entity vis-a-vis the organization. For the purpose of our exposition, we do not need to be exhaustive. We propose for now the following: $type\_role\_IO \in \{None, UX\_researcher, UX\_designer, AI\_researcher, AI\_developer, engineer, product\_manager, legal, governance, other\}$
\fanny{added "other". I couldn't easily model the relationship with HF folks or SN partners like Deloitte/Accenture}
        \item \agathe{There could be other types of relations between individuals and organizations. TBD what we do with that when we get to the supply chain relations and "beliefs".}
         \item \textbf{Relations within each human entity type}: $R\_I: I \times I \times \{type\} \rightarrow True/False$, $R\_O: O \times O \times \{type\} \rightarrow True/False$ respectively.\\ 
These relations are reflexive and symmetric, but not transitive. For simplification, we do not specify the type of relation, as it is not important for the exposition of our work. 
\TODO{define $\{type\}$, because intuitively i (fanny) thought it couldn't be ref or sym}
\fanny{Proposal for $\{type\}$:
\begin{itemize}
    \item individuals: $R_I = \{authority, collaborator, stakeholder, other\}$ (cross-ref with the excel sheet)
    \item organizations: $R_O = \{provider, partner, competitor, collaborator, other\}$
\end{itemize}
ISSUE: some rel types are directional, unsure how valuable it is at this point. Potential to leverage for trust relations or just annoying/redundant? If the latter, refine.}
    \end{itemize}
    \item \textbf{Relations between individual entities and technical artifacts}: $R\_ITA: I \times TA \times type\_ITA \rightarrow True/False$\\
    The type the relation can take corresponds to the type of relation the individual has vis-a-vis the system.
        We propose $type\_ITA = \{impactor, user, potentially\_impacted, public, auditor, other, None\}$
        \fanny{added "auditor" and "other": the latter may be part of impactor/producer though: i'm thinking of projects we transfer to ppl but they don't really work on it.}
    \item \textbf{Relations between organizational entities and technical artifacts}:  $R\_OTA: O \times TA \times type\_OTA \rightarrow True/False$\\  
    The type the relation can take corresponds to the type of relation the organization has vis-a-vis the system. 
        We propose $type\_OTA = \{developer, deployer, assessor, user, potentially\_impacted, public, other, None\}$
        \fanny{added "other": i'm thinking of open-source models that are not maintained but still on HF hub}
\end{itemize}
}


\subsubsection{The AI Supply Chain is Complex}
Note that the AI supply chain and the interactions between entities across the chain are complex. Our formalization above allows us to account for the main complexities we identified in our interviews. Note however that the formalization lacks some obvious constraints about the entities --we do not specify them exhaustively for space considerations. Here, we simply illustrate some of the constraints and highlight major complexities, for a reader who would like to extend our formalization for their own study.

\paragraph{Obvious constraints}
\fanny{for improved readability, constraints/propositions should be near definitions so we can more easily make sense of them}
%Additional constraints: The objective of our work is not to specify in extensive detail the different entities and relations. Yet, we would like to warn the reader (who might want to use our framework) of the existence of additional, obvious, constraints and implications from the relations between the human entities and technical artifacts based on their types. For brevity, we do not describe them further here.
The first type of constraint revolves around minimum requirements for the existence of instantiated entities. Naturally, for an AI system to exist, both a minimum number of technical artifacts should have been developed, and a minimum set of human entities should have developed those. 
For instance, for any technical artifacts of type system, one can assume that there exists at least one organization for each of the possible types in the relation $R\_OTA$, while for technical artifacts of type ``other'', there is at least one organizational entity for ``developer'', ``assessor'', ``deployer'', ``user'' (with the last two having the same meaning) --the public might not directly be aware and related to an AI component, and not all AI components might affect populations directly (e.g., the data processing pipeline does not necessarily affect anyone directly). 
\agathe{To discuss with everybody: that could be contestable in a way?}
If we then consider the relation between organizational entities and individual entities, naturally an organization is made of humans. Hence, there is always at least one instance of individual entity connected to the instance of an organizational entity via the relation $R\_IO\_role$ with a type non-None.
\fanny{what do we do with org that are no longer active and released whatever an open source model avail? }

The second type of constraint revolves around the interplay of entity and relation types across the technical artifacts and human entities. 
For instance, if an individual entity has the type ``impactor'' vis-a-vis an AI system, then this individual entity should be related to an organization that has a type ``developer'', ``deployer'', or ``assessor'' of the same AI system, and this $R\_IO\_role$ relation should be characterized by a non-"None" type.
\fanny{contre-exemple: community-led dev w/ independant researchers like big code. I think that the following holds:
Let $o \in O$ and $ta \in TA$ such that org role is <ORGROLE>, then there exists $i \in I $ such that <INDROLE>.}


\subsection{Trust relations}


\subsubsection{Basic Relations}

Now that we have formalized the important components of an AI supply chain, we formalize trust relations across components, still based on the observations we made in our interviews. 

\framedtext{
\underline{Formalization of trust relations:}
\begin{itemize}[leftmargin=*]
\item The space of activities: A; instantiation of activity: $a_x \in A$
\item The type of activity: $type\_A \in \{None, other, R\_ATA(A \times TA)\}$
\begin{itemize}
    \item An activity can have only one type.
    \item Some activities are directly related to an AI system while others are not. In the case an activity is ``None'', it means that there is no activity at all. This is important within the trust relation since not all trust relations require an activity.
\end{itemize}
\item \agathe{We might specify further later the types of activities}
\item Trust relation: 
% $TR(\{I, O\}, \{I, O, TA\}, A) \rightarrow (trust\_extent, trust\_warrantedness)$
\begin{align*}
    TR : I \cup O \times I \cup O \cup TA \times A &\to [0,1] \times [0,1] \\
    (truster, trustee, activity) &\mapsto (extent, warrantedness)
\end{align*}
\TODO{Is it independant?}
\agathe{from fanny: is warrantedness $\{0,1\}$?}
\end{itemize}
}


\subsubsection{Factors}
Factors impact the trust relation.

\framedtext{
\underline{\textbf{Formalisation of the factors that impact the trust relation:}}
\begin{itemize}[leftmargin=*]
    \item Trust factors: F(TR(trustor, trustee, activity)); F(TR(trustor, trustee, activity)) $\rightarrow$ TR(trustor, trustee, activity)
    \fanny{could be $\implies$}

    \item List of factors:
    \begin{itemize}
        \item Characteristics of the trustor
        \item Trust cues built on top of the characteristics of the trustee
        \item Contextual factors:
        \begin{itemize}
            \item Chained trust
            \item Other contextual information related to the activity at hand
            \item Other contextual information not related to the activity at hand
        \end{itemize}
    \end{itemize}
\end{itemize}
}



\subsubsection{Formalizing the chains of trust}
\fanny{Do we still use $TR$ which outputs 2 values? Assuming we consider trust is a spectrum, it's complicated to interpret the axioms below. Correlation is an avenue: i like that it remains a spectrum rather than binary (as it feels now).}

We will note the belief of the trustor of the interest as \textit{Belief(Relation)}.
Note that we have for now focused on the trustor and their belief. Naturally, these beliefs are themselves impacted by contextual factors, and among them are beliefs of other trustors. While we do not represent these in our modelisation, this means that the belief relation should in the future specify which human entities it relates to, and account for the contextual factors that impact it.

In order to formalize the chained trust that impacts the final trust relation, we first need to describe a few axioms that makeup trust relations. Note that we enounce these axioms in a very simple manner, yet one should not neglect that the impact of a trust or belief relation on another is not as simple as represented: it varies across trustors and trustees depending on many contextual factors. 
These axioms can then be chained in order to create a chain of trust. 

\fanny{We should define properly the Belief and Relation first. Comments are based on my intuition.}

\framedtext{
 \underline{\textbf{Formalization of the chained trust:}}
 Let $e_1 \neq e_2 \neq e_3 \in I \cup O$ and $a_1 \neq a_2 \in A$.
 \fanny{I assume that trust is a spectrum here (see $TR$ def above). What can't we simply use $TR$ instead of TR1 and TR2?}
\begin{itemize}[leftmargin=*]
    \item Trust axioms (to simplify the notations, we note $e\_x$ any entity (either individual or organizational). 
    % \fanny{are the axioms correct? can we express them better? are we missing any axiom?}
    \begin{itemize}
        \item Trustee impact: if TR1(e1, e2, a1) and (e1 != e3, e2 != e3), then TR2(e1, e3, a1) \\
        \fanny{$TR(e_1, e_2, a_1)$ and $TR(e_1, e_3, a_1)$ are correlated? abuse of terminology bc $TR$ isn't define as a random variable but proportional feels too restrictive.}
        If a trustor trusts a trustee to be able to conduct a certain activity, they are more likely to also trust other trustees to conduct the same activity.
        \fanny{Should we frame it with a transitivity lens instead?}
        \item Activity impact: if TR1(e1, e2, a1) and a1 != a2, then TR2(e1, e2, a2)  \\
        \fanny{$TR(e_1, e_2, a_1)$ and $TR(e_1, e_2, a_2)$ are correlated? }
        If a trustor trusts a trustee to conduct a specific activity, they are potentially likely to trust the same trustee to conduct another activity (this activity might be None and they might simply trust the trustee overall).
        \item Trustee-composition: if TR1(e1, e2, x) and TR2(e1, e3, x) and belief(relation(e4: e2, e3)), then TR3(e1, e4, x)\\
        \fanny{Current statement: redundant with the first axiom bc the activity is constant across the board. From the text below, i understand that this is independent from the activity, so i would use $x, y, z \in A$ instead.}
        If a trustor trusts two different trustees that are related by a relation that includes a fourth entity, then the trustor is likely to also trust this last entity. This is especially the case when talking about different components of the same AI system, or when talking about several individual entities working for the same organizational entity. \agathe{Fanny: this one seems to be a sub-axiom of the last one, right? if so, maybe we don't need it but just use it as an example later.}
        \item Trustee-transitivity: if TR1(e1, e2, a1) and belief(relation (e2, e3, a2)), then TR3(e1, e3, a1) \fanny{redundant again with first axiom}
    \end{itemize}
    \item ChainOfTrust(e1, e2, a1): one valid path \fanny{}
    \item ChainedTrust(e1, e2, a1): the set of paths \fanny{}
\end{itemize}
}

trust and canonical properties of chains

\agathe{note:take inspiration from \cite{suresh2021beyond} to evaluate our framework (sec. 4)???}


